Detecting Unintended Memorization in Language-Model-Fused ASR

End-to-end (E2E) models are often being accompanied by language models (LMs) via shallow fusion for boosting their overall quality as well as recognition of rare words. At the same time, several prior works show that LMs are susceptible to unintentionally memorizing rare or unique sequences in the training data. In this work, we design a framework for detecting memorization of random textual sequences (which we call canaries) in the LM training data when one has only black-box (query) access to LM-fused speech recognizer, as opposed to direct access to the LM. On a production-grade Conformer RNN-T E2E model fused with a Transformer LM, we show that detecting memorization of singly-occurring canaries from the LM training data of 300M examples is possible. Motivated to protect privacy, we also show that such memorization gets significantly reduced by per-example gradient-clipped LM training without compromising overall quality.

==> unused/revised_intro.tex <==
\section{Revised Introduction}
\label{sec:rev-intro}

In this work, we make three main contributions to answering the above question, using as our testbed a production-grade Conformer RNN-T acoustic model with a Transformer LM:

Our first contribution is to design a framework to test for unintended memorization using only a query access to the ASR system. We do this by inserting a set of random ``canaries'' into the LM's training data, and observing the resulting model's performance on these examples. We need to overcome a pair of obstacles: First, since the ASR model accepts audio and not text, we use a Text-To-Speech (TTS) system to generate synthetic utterances for querying the ASR system. Next, unlike conventional attacks on LMs which require the use of a confidence score, e.g.~perplexity, ASR systems typically only give the single top transcript for a given audio sequence. Thus, we use the model's WER on canaries versus baseline examples as our primary metric.

We test for memorization across a range of canary frequencies and LM capacities. Our results show that memorization is detectable even for canaries that appear only once in a large (300M sample) training corpus, and then grows significantly the more frequently a canary is repeated in the training data (from 1 to 32 times). We also show how increasing model capacity leads to increased memorization.

Our next contribution is to study the effect of per-example gradient clipping on mitigating memorization, an idea motivated by prior work~\cite{CLEKS19, TRMB20}. Our experiments here demonstrate that this technique can significantly reduce the level of memorization without appreciable loss of overall utility in the model.

Finally, we observe that while using \emph{clean} TTS utterances can be useful for detecting memorization, there can be instances where the ASR system may not leverage the LM for providing the top transcripts, e.g.,~if the TTS utterances are   easy to predict for the AM itself.
In such cases, the LM's memorization may not be able to surface to the top transcript predictions which we use for inference.
Thus, we add noise to parts of the TTS utterances such that the LM's predictions can be leveraged by the ASR system.
Moreover, we design a simple classifier that can use the top transcripts for these utterances to conduct a \emph{membership inference} task.
We provide an analysis of how metrics like precision and recall (commonly used for evaluating membership inference attacks) can be used to demonstrate the extent of unintended memorization in ASR LMs.
For instance, we show in our experiments that while our classifier shows a baseline (50\% precision, 13\% recall) for non-memorized sequences of data, it achieves ($\sim$80\% precision, $\sim$50\% recall) for sequences that appeared only eight times among 300M other samples for LM training and were subsequently memorized.
